3D-GIF: 3D-Controllable Object Generation via Implicit Factorized Representations

While NeRF-based 3D-aware image generation methods enable viewpoint control, limitations still remain to be adopted to various 3D applications. Due to their view-dependent and light-entangled volume representation, the 3D geometry presents unrealistic quality and the color should be re-rendered for every desired viewpoint. To broaden the 3D applicability from 3D-aware image generation to 3D-controllable object generation, we propose the factorized representations which are view-independent and light-disentangled, and training schemes with randomly sampled light conditions. We demonstrate the superiority of our method by visualizing factorized representations, re-lighted images, and albedo-textured meshes. In addition, we show that our approach improves the quality of the generated geometry via visualization and quantitative comparison. To the best of our knowledge, this is the first work that extracts albedo-textured meshes with unposed 2D images without any additional labels or assumptions.

==> 1_intro_before.tex <==
\section{Introduction}
\label{sec:intro}

Generating photo-realistic images has been a long-standing problem in computer vision.
Addressing this concern, generative adversarial network (GAN) has drawn attention for its capability of generating high-quality images with novel contents.
Albeit the success of GAN, the generated images are still locked in 2D.
Since they are not able to disentangle the 3D factors from the contents, there still remain limitations in content creation and image editing in 3D space (\eg viewpoint modification, re-lighting, etc.).
To enhance 3D controllability, 3D-aware image synthesis\cite{} has been proposed, employing 3D representations such as voxel~\cite{} and implicit functions~\cite{}.
Among them, several approaches~\cite{} have successfully controlled the viewpoints while preserving the image quality and multi-view consistency, by utilizing neural radiance fields (NeRF).
Also, they present the ability of 3D geometry extraction from generated volume density using the marching cube algorithm.

However, as shown in Fig.~\ref{fig:intro_failure}, the extracted 3D geometry obtained from the existing state-of-the-art model (pi-GAN) presents unrealistic quality, while the model generates realistic 2D images at different viewpoints.
% view dependent color나 모델이 light를 알고있는게 multiview에서 realistic하지만 unrealisitc한 geometry를 가질 수 있게하는 거 설명
% Accordingly, it is difficult to force the model to learn the accurate 3D geometry without separately considering light condition during the training.
This is due to the fact that realistic multi-view images can be projected from unrealistic 3D geometry under certain view directions and light conditions. %with certain view direction and light condition.
% different realistic color depending on views even though the geometry is unrealistic.

We demonstrate this problem with a toy example presented in Fig.~\ref{fig:intro_sphere}.
The second row of Fig.~\ref{fig:intro_sphere} shows the images projected from a dented sphere with different viewpoints and light conditions in the first row.
As shown in the first and the second column, there are cases where we cannot distinguish the dent of its corresponding geometry even with the images projected from two different view directions.
Accordingly, being able to generate realistic multi-view images does not necessarily guarantee the desired corresponding geometry. 
Also, the previous approaches predicts view-dependent color to represent non-Lambertian effect.
This exacerbates the above problem since the model is allowed to predict the different color that makes the projected 2D image realistic at the given viewpoint even though the geometry is unrealistic.


Meanwhile, as in the third column, we can easily detect unrealistic geometry by changing the light direction.
With this insight, we propose a method to generate a volume representation with realistic geometry as follows:
1) To disentangle the light condition when generating images, our model learns factorized volume representations (\ie albedo, normal vectors, specular parameters) that are independent of the viewpoints and light conditions, instead of the view-dependent color output of previous methods.
2) We train the model with sampled light conditions to force realistic multi-view image generation via photometric reconstruction (\ie ambient, diffuse, and specular reflection) under arbitrary light conditions.  % under arbitrary light condition. multi-view and multi-light
3) We update volume density to reflect light-consistent geometry property (\ie normal) learned from above.

% To address this issue, we first obtain light-consistent geometry property which can generate realistic multi-view images under arbitrary light condition.
% Then, improve 

% weak supervision of geometry obtained from training the model with the physical prior and disentangled light condition. 
% and this makes the model generate realistic volume representation as well as 2D images.


In this way, our approach achieves more realistic geometry of generated representation than the previous 3D-aware image generation methods.
To demonstrate the effectiveness of our model, we conduct quantitative and qualitative experiments using three different un-posed single-view image datasets, CelebA, Cats, and BFM. 
% According to the results, our method generates more realistic geometry compared to the existing methods.
% Also, our model allows for re-lightable images and 3D textured mesh from the generated implicit representation, since our model disentangle the light reflection and predicts view-independent volume representation. 
Since our model predicts view-independent density, albedo, normal, specular parameters, we are able to generate viewpoint controllable, re-lightable images and also re-lightable 3D textured mesh.

We summarize our contributions as follows:
\begin{itemize}[noitemsep,topsep=0pt]
    \item We present MODEL that generates 3D implicit representation disentangled into albedo, normal, and specular parameters trained only with single-view images (without any additional labels and assumptions).
    \item We successfully combine physical reflection prior, which improves the geometry of generated 3D objects.
    \item We are the first to generate re-lightable textured 3D meshes only using single-view 2D images. % + re-lightable images
    % \item We achieve the state-of-the-art performance on 3D-aware image synthesis from unsupervised 2D data.
\end{itemize}


\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/intro_failure.png}
    \vspace{-0.7cm}
    \caption{An example of failure cases of the existing SOTA method.}
    \label{fig:intro_failure}
    \vspace{-0.5cm}
\end{figure}
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/intro_sphere_ex_ppt_2.png}
    \vspace{-0.7cm}
    \caption{Toy example.}
    \label{fig:intro_sphere}
    \vspace{-0.5cm}
\end{figure}

% based on the learned geometry property (\ie normal)
% 이러한 insight를 가지고 우리는 다음과 같은 방법으로 realistic환 geometry를 갖는 volume representation을 생성하는 방법을 제안한다.
% 1) light condition과 모델을 disentangle하여 임의의 light condition에 대하여 realsitic한 photometric reconstruction(i.e. ambient, diffuse, and specular reflection)을 만족하는 volume parameter(i.e. albedo, specular parameter, normal)를 학습한다.
% 2) 앞에서 구한 geometry의 특성 (i.e. normal)에 맞도록 volume density를 업데이터하여 realistic한 geometry를 강제한다.
% 즉, light reflexction이 geometry에 따라 어떻게 일어나는지에 대한 physical prior를 모델에 제공하여 우리는 geometry에 대한 weak supervision을 획득할 수 있고, 이는 2D image 뿐 아니라 geometry가 realistic한 volume representation을 생성하도록 한다.


% 따라서 우리는 모델이 임의의 light에 대하여 realistic한 이미지를 만들 수 있도록 light를 sampling했고 generative 모델에 geometry에 따라 light reflection (\eg ambient, specular, and diffuse)이 어떻게 일어나는지에 대한 physical prior를 직접적으로 제공하여 보다 realistic한 3D geometry를 생성하는데 성공하였음.
% %기존 3D-aware image generation 모델들은 생성된 2D 이미지를 realistic 하게 만드는 것만을 학습하지만 
% 우리의 proposed 모델은 geometry 특성 (pred normal) 과 light에 의한 reflection효과를 고려하여 이미지를 생성하고, 이러한 특성이 geometry에 반영되도록 강제하기때문에 projection 된 2D 이미지 뿐만 아니라 3D geometry도 realistic하게 생성할 수 있음.
% 또한 view-independent한 density, albedo, normal, specular parameter를 예측하기 때문에 viewpoint controllable 뿐 아니라 re-lightable한 이미지, re-lightable 3D textured mesh를 생성할 수 있음.

% Accordingly, it is difficult to force the model to learn the accurate 3D geometry without separately considering light condition during the training.
% 만일 모델이 찌그러진 구를 생성했다면 projection된 이미지도 구의 형태와 거리가 멀어야 모델이 implicit하게 구의 형태를 보정하는 loss를 흘려줄 수 있게된다.
% Figure 3는 viewpoint와 light condition을 바꿔가며 찌그러진 sphere 매쉬를 주어진 view point 로 projection한 이미지를 확인한 것임.
% Figure 3는 찌그러진 sphere 매쉬를 다양한 viewpoint, light condition에서 projection된 이미지를 확인한 것임.
% geometry가 구형태가 아님에도 불구하고 projection 된 이미지에서 구를 바라본 것 처럼 보이는 경우가 존재함. (첫번째, 두번째 컬럼)
% Geometry가 unrealistic하더라도 multiview에서 realistic해보이는 경우가 존재함. (첫번째, 두번째 컬럼)
% 이렇기 때문에 3d representation으로부터 생성된 2D image가 realistic하다는 것이 해당 물체의 Geometry가 realistic함을 보장하지 않는다는 걸 알수있음.
% 이렇기 때문에 생성된 2D image의 quality 혹은 reality가 Geometry가 realistic함을 보장하지 않는걸 알수있음.
% emjay : 삭제?
% 이러한 경우는 모델이 unrealistic한 geometry를 생성하게 됨.
% emjay : 삭제?
% 이런 unrealistic한 geometry를 가지고는 3D application에 다양하게 활용하기 어려움.

% %%% Disentanglement of the 'light' from the shape or color is necessary
% 세번째 컬럼과 같이 빛 방향을 바꾼다면 쉽게 unrealitic한 geometry를 감지할 수 있다. 
% 이러한 insight를 가지고 우리는 다음과 같은 방법으로 realistic환 geometry를 갖는 volume representation을 생성하는 방법을 제안한다.
% 1) light condition과 모델을 disentangle하여 임의의 light condition에 대하여 realsitic한 photometric reconstruction(i.e. ambient, diffuse, and specular reflection)을 만족하는 volume parameter(i.e. albedo, specular parameter, normal)를 학습한다.
% 2) 앞에서 구한 geometry의 특성 (i.e. normal)에 맞도록 volume density를 업데이터하여 realistic한 geometry를 강제한다.
% 즉, light reflexction이 어떻게 일어나는지에 geometry에 따라 어떻게 발생하는지에 대한 physical prior를 모델에 제공하여 우리는 geometry에 대한 weak supervision을 획득할 수 있고, 이는 2D image 뿐 아니라 geometry가 realistic한 volume representation을 생성하도록 한다.
% % 매쉬랑 re-light 얘기



%%% Advances in computer graphics - which requires human in the loop since it cannot create contents on its own
% 이전: Graphics technique이 movies나 gaming 등 다양한 분야에서 impressive한 results를 보여주고 있지만 contents creation을 위해서 많은 사람의 노동력을 필요로 한다는 문제를 지님.
% Computer vision에서는 high-quality의 photo-realistic한 이미지를 생성하는 문제가 오래된 문제로 자리잡고 있다.
% \textcolor{red}{Generating high-quality and photo-realistic images has been a long-standing problem in computer graphics.}
% \textcolor{red}{Recent advancements in computer graphics have significantly enhanced the quality of scenes in movies and games.}
% \textcolor{red}{However, those techniques .}
%%% GAN which is capable of generating photo-realistic images with novel contents?
% 이에 대한 대안으로 딥러닝이 부상하고 있으며 특히 GAN이 photo realistic한 고해상도 이미지를 생성하며 성공적인 모습을 보여주고 있음.
% \textcolor{red}{Addressing this concern, generative adversarial networks (GAN) has drawn attention for its capability of generating high-quality and photo-realistic images with novel contents.}
%%% GAN generated images are still locked in 2D images - extension to 3D space + controllable attributes
% GAN이 photo realistic한 고해상도 이미지를 생성하며 성공적인 모습을 보여주고 있음.
% \CY: Controllable image synthesis extends the application in content creation and image editing.
% \CY: 이미지 생성에 controllability를 추가 하는 연구가 활발히 진행되고 있지만, 3D 요소를 고려하지 못한다는 한계를 지닌다.
% 그러나 realistic한 2D 이미지를 생성하는 것만으로는 특정 application (novel view synthesis 등) 에 한계를 지니기 때문에 이미지 생성에 controllability를 추가 하는 연구가 활발히 진행되고 있음.
% \textcolor{red}{Albeit the success of GAN, there still remain limitations as follows; 1) attributes of contents are usually not controllable or manipulable, and 2) generated contents are still locked in 2D.}
% \textcolor{red}{To overcome the former drawback, several work has proposed controlling the latent vector to manipulate the attributes on images.}
% latent vector를 조절하여 이미지를 control하는 work들이 있지만 사후처리로 latent의 방향을 구해야 한다는 단점이 있고 3D 요소를 고려하지 않기 때문에 3D shape과 viewpoint를 disentangle 하는 것에 어려움이 있음.
% \textcolor{red}{However, those approaches require post-processing to obtain the direction of latent vectors, and most of all, they cannot address the later problem, generating contents in 3D-aware manner.}
% \textcolor{red}{Being locked in 2D makes it more challenging for the methods to disentangle the 3D shape of contents from the viewpoint.}
% 이에 따라 3D representation (\eg voxel and implicit function)을 활용한 3D aware-image synthesis work들이 발전함.
% \textcolor{red}{Therefore, 3D-aware image synthesis\cite{} has been proposed, employing 3D representations such as voxel~\cite{} and implicit functions~\cite{}}
% 특히 Neural Radiance Field 기반의 generative 모델이 image quality나 multi view consistency 유지하며 viewpoint control에 성공함.
% \textcolor{red}{Among them, several approaches~\cite{} have successfully controlled the viewpoints while preserving the image quality and multi-view consistency, by utilizing neural radiance fields (NeRF).}
% 또한 marching cube를 이용하여 3D geometry를 2D image에서 분리하여 생성하는 모습을 보여줌.

% 원래 한글
% Computer vision에서는 high-quality의 photo-realistic한 이미지를 생성하는 문제가 오래된 문제로 자리잡고 있다.
% GAN이 photo realistic한 고해상도 이미지를 생성하며 성공적인 모습을 보여주고 있음.
% \CY: Controllable image synthesis extends the application in content creation and image editing.
% \CY: 이미지 생성에 controllability를 추가 하는 연구가 활발히 진행되고 있지만, 3D 요소를 고려하지 못한다는 한계를 지닌다.
% 그러나 realistic한 2D 이미지를 생성하는 것만으로는 특정 application (novel view synthesis 등) 에 한계를 지니기 때문에 이미지 생성에 controllability를 추가 하는 연구가 활발히 진행되고 있음.
% 그러나 Figure 2에서 보듯 기존 SOTA 모델이 2D image는 photo realistic하게 생성하지만 3D geometry를 확인하면 unrealistic하게 생성하고 있음.


%%% Limitation of previous state-of-the-art methods in novel-view synthesis - Quality of 2D generated images vs Quality of their corresponding 3D meshes
% 그러나 Figure 2에서 보듯 기존 SOTA 모델이 2D image는 photo realistic하게 생성하지만 3D geometry를 확인하면 unrealistic하게 생성하고 있음.
% 해답이 여러개 realistic 한거 찾기
% emjay : 기존의 방법은 view dependent한 color를 사용하고있기 때문에 multi view에서 2D image를 realstic하게 만들더라도 3D geometry가 unrealstic할 수 있음.
% Single view images만을 이용하여 3D geometry를 학습하는 것은 ill-posed problem이기 때문에 multi view에서 2D image를 realstic하게 만들더라도 3D geometry가 unrealstic할 수 있음.% (optional) 그리고 이는 다양한 3D application에 한계를 지니게 함.




% 따라서, 다음과 같은 방법으로 빛을 disentangle하여 모델을 학습하면 realistic한 geometry를 생성하도록 강제할 수 있다.



% 1) 먼저 임의의 light condition에 대하여 realistic한 photometric reconstruction을 만족하는 geometry 특성 (\eg normal)을 구해낼 수 있고, 
% %emjay 2) 앞에서 구한 normal을 만족하도록 volume density (sigma)를 업데이트하여 해당 sigma로 부터 얻어진 geometry가 realistic해지도록 강제할 수 있다. 
% 2) 이어서 앞에서 구한 geometry의 특성에 맞도록 volume density (sigma)를 업데이트하여 realistic한 geometry를 강제할 수 있다. 
% % emjay 왜 weak supervision?
% 따라서 임의의 light에 대해서 이미지를 realisic하게 만들 수 있는 normal을 구하고 이를 geometry의 weak supervision으로 사용하여 geometry를 realistic하게 만듦

% 학습시 세번째 컬럼과 같이 빛 방향을 임의적으로 바꿨을 때도 realistic한 geometry를 생성하도록 강제한다면, 위의 문제를 해결할 수 있을 것이다.
% 따라서 우리 모델은 빛을 임의로 바꿔가며 unrealitic한 geometry를 감지하고, 이 경우에도 realistic한 geometry를 생성하도록 강제하는 식으로 학습을 진행한다...


% 이를 해결하기 위해서는 빛 요소를 모델과 disentangle 하여 어떤 빛아래에서도 realistic한 geometry를 생성할 수 있도록 해야한다.
% 따라서 우리는 세번째 컬럼과 같이 빛 방향을 임의적으로 바꿔가며 unrealitic한 geometry를 감지하고, 

% 그렇기 때문에 빛을 모델과 disentangle하여 모델을 학습하면 realistic한 geometry를 생성하도록 강제할 수 있음. 

% 세번째 컬럼과 같이 빛 방향을 바꾼다면 쉽게 unrealitic한 geometry를 감지할 수 있음.


% 추가적인 라벨 없이 single-view 2D 이미지만을 활용하여 3D textured mesh를 최초로 성공적으로 생성하였음.


% GAN이 photo realistic한 이미지를 생성하는데 성공적인 모습을 보여옴.
% % 필요성이 들어가거나 하이레벨에서 먼저 쓰고 조금 더 좁혀가는 식의 문장 필요
% 그러나 실제 세상이 3D라는 점을 고려하지 않기 때문에   3D shape과 viewpoint를 disentangle 하는 것에 어려움이 있음. 
% % multiview synthesis와 같은 3d application 하나정도 써주고 이런거 못한다는식으로 ... 이렇게 3D geometry가 망가지면 3D application에 제대로 활용을 할수가 없음 
% 이에 따라 3D aware-image synthesis work들이 발전함.
% 특히 Neural Radiance Field 기반의 generative 모델이 image quality나 multi view consistency 측면에서 성공적인 모습을 보여줌.
% 그러나 Single view images만을 이용하여 3D Object를 생성하는 모델을 학습하는 것은 strongly ill-posed problem이기 때문에 multi view에서 2D image를 realstic하게 만들더라도 3D geometry가 unrealstic할 수 있음.
% Figure 2에서 보듯 기존 SOTA 모델들이 2D image는 photo realistic하게 생성하지만 생성된 3D geometry를 보면 unrealistic하게 생성하고 있음. %(pi-gan 논문에서 직접적으로 언급함)

% % geometry에 따라 light reflection이 어떻게 영향을 받는지
% % 왜냐하면 이런 mesh에 light를 달리했을때 (Figure 3의 세번째 컬럼을 참고하면 ) 바로 망가지는 것을 볼 수 있음.
% Figure 3에 있는 toy example을 보면 sphere 매쉬가 찌그러져 있지만 첫번째, 두번째 컬럼과 같은 viewpoint, light condition의 경우에 projection된 이미지는 자연스러운 circle이 나옴
% 그러나 빛의 방향을 바꾼 세번째 컬럼의 경우에는 projection된 이미지가 unrealistic 해지는 것을 확인 할 수 있음
% %%%%%%%%%실험추가%%%%%%%%%%%
% % 원래 figure2 비슷한 사진 넣고
% % 정상적인 구, 반대로 파인 구 매쉬 넣고
% % 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 우리는 generative 모델에 geometry에 따라 light reflection이 어떻게 일어나는지에 대한 physical prior를 직접적으로 제공하여 보다 realistic한 3D geometry를 생성하는데 성공하였음.
% % geometry에 따라 light reflection이 어떻게 일어나는지에 대한 physical priror라는 단어를 쓸지 아니면 photometric reconstruction을 쓸지 고민
% 기존 3D-aware image generation 모델들은 생성된 2D 이미지를 realistic 하게 만드는 것 만을 학습하지만 우리의 proposed 모델은 
% % light reflection과 albedo를 disentangle하고, 
% geometry와 light direction change에 dependent한 reflection효과를 고려하여 이미지를 생성하기 때문에 projection 된 2D 이미지 뿐만 아니라 3D geometry도 realistic하게 생성할 수 있음.
% %  
% % 즉, 기존 모델은 3D geometry에 직접적인 영향을 주는 loss가 없었지만 우리는 있게 만든것
% 또한 albedo, normal, specualr parameter를 예측하기 때문에 viewpoint controllable 뿐 아니라 re-lightable한 이미지를 생성할 수 있음.
% 또한 view independent한 volume과 albedo를 예측하기 때문에 marching cube 알고리즘을 이용하여 re-lightable 3D textured mesh를 생성할 수 있음.
% 추가적인 라벨 없이 single-view 2D 이미지만을 활용하여 3D textured mesh를 최초로 성공적으로 생성하였다.





%%%%%%%%%%%%%%%%% 이전 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The 3D gaming and graphics industries are moving towards automatic content generation techniques.
% Several studies aim to generate 3D objects.
% However most of the existing 3D object generation work need 3D parametric models or 3D ground truth which are expensive to collect.
% Some work targets to learn inherent 3D information in an unsupervised manner with only using 2D images, but they can only generate viewpoint controllable 2D images.
% We aim to generate 3D object (\eg, textured mesh) with only using single-view 2D images.

% We summarize our contributions as follows:
% \begin{itemize}[noitemsep,topsep=0pt]
%     \item This is the first work that successfully generates re-lightable textured 3D meshes with using only single-view 2D RGB images.
%     \item We propose factorizable generative NeRF, which successfully disentangles texture into albedo, normal, and specular.
%     \item Our model successfully predicts object volume occupancy and object/background probability at 3D-point-level.
%     \item We achieve the state-of-the-art performance on 3D-aware image synthesis from unsupervised 2D data.
% \end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------------------------------------------------------------

% {
% 찌그러진 sphere 매쉬를 다양한 viewpoint, light condition에서 projection된 이미지를 확인한 것임.
% 첫번째 컬럼과 두번째 컬럼에서 보이듯 viewpoint를 바꾸었음에도 불구하도 projection된 이미지는 완벽한 구를 projection한것과 차이가 없음. 이는 모델이 부자연스러운 3D 모델을 생성하더라도 적절한 빛의 방향을 설정하여 2D project상에서 자연스럽게 만들어 버리기 때문이다. 따라서 이렇게 해당 빛 방향에 대해서 자연스러운 3D model은 3번째 열과 같이 다른 방향에서 빛을 비추게 되면 즉시 부자연스러워진다. 이 때문에 빛을 disentangle하여 3D 생성 모델에서 빛에 대한 dependency를 없애게 된다면 모델은 모든 방향의 빛에 대해서 최적화를 해야만하므로 더욱 자연스러운 3D 모델을 생성할 수 있다. 
% }






% 그러나 realistic한 2D 이미지를 생성하는 것만으로는 application (e.g. novel view synthesis 등) 에 한계를 지니기 때문에 이미지 생성에 controllability를 추가 하는 연구가 활발히 진행되고 있음.
% latent vector를 조절하여 이미지를 control하는 work들이 있지만 사후처리로 latent의 방향을 구해야 한다는 단점이 있고 3D 요소를 고려하지 않기 때문에 3D shape과 viewpoint를 disentangle 하는 것에 어려움이 있음.
% 이에 따라 3D representation (e.g., voxel, implicit function)을 활용한 3D aware-image synthesis work들이 발전함.
% 특히 Neural Radiance Field 기반의 generative 모델이 multi view consistency 유지하며 high quality의 viewpoint controlable image generation에 성공함.
% 또한 marching cube를 이용하여 3D geometry를 disentangle 하여 생성하는 모습을 보여줌.

% 그러나 Figure 2에서 보듯 기존 SOTA 모델이 2D image는 photo realistic하게 생성하지만 생성된 geometry를 확인하면 unrealistic하다는 것을 확인할 수 있음.
%single view images만을 이용하여 3D geometry를 학습하는 것은 ill-posed problem이기 때문에 3D representation의 geometry가 unrealistic하더라도 multi view consistency와 resalisic을 만족시킬 수 있다.
% Figure 3의 toy example (a), (b)에서 볼 수 있듯, dented sphere가  다양한 viewpoint에서 projection된 이미지가 realistic한 shphere과 같은 것을 확인 할 수 있다.
% 이러한 경우는 모델이 realistic한 geometry를 생성하도록 강제할 수 없다.
% 그러나 이러한 경우는 (c)와 같이 light를 disentangle한다면 unrealisitc한 geometry를 쉽게 감지할 수 있고 arbitrary light에 대해서 생성한 이미지가 realistic 하도록 강제하면 geometry를 realistic하게 만들 수 있다.
% 따라서 우리는 light을 모델과 disentangle하고 임의의 light에 대해서 이미지를 realistic하게 만들 수 있는 
% 따라서 임의의 light에 대해서 이미지를 realisic하게 만들 수 있는 normal을 구하고 이를 geometry의 weak supervision으로 사용하여 geometry를 realistic하게 만듦 


% 따라서 우리는 light를 외적으로 분리하고 generative 모델에 geometry에 따라 light reflection이 어떻게 일어나는지에 대한 physical prior를 직접적으로 제공하여 보다 realistic한 3D geometry를 생성하는데 성공하였음.
% 기존 3D-aware image generation 모델들은 생성된 2D 이미지를 realistic 하게 만드는 것 만을 학습하지만 우리의 proposed 모델은 geometry와 light direction에 dependent한 reflection효과를 고려하여 이미지를 생성하기 때문에 projection 된 2D 이미지 뿐만 아니라 3D geometry도 realistic하게 생성할 수 있음.
% 또한 view independent한 density, albedo, normal, specular parameter를 예측하기 때문에 viewpoint controllable 뿐 아니라 re-lightable한 이미지, re-lightable 3D textured mesh를 생성할 수 있음.


%%% Method 에 아래 내용 추가
% 1. As also pointed out in nerfactor, model normal이 noisy하기 때문에 model normal을 바로 reconstruction에 사용하기 힘들다. 
% 2. 우리가 사용하는 모든 components (albedo, specular, normal) 은 sigma에 의해 volume rendering 되기 때문에, sigma의 x에서의 gradient값을 직접 normal로서 사용하면 학습이 불안정하다.
% 따라서, 우리는 안정된 학습을 위해 regression branch를 추가하여 realistic한 photometric reconstruction을 만족하는 normal을 구하도록 했고, 해당 normal을 이용하여 sigma값을 업데이트하여 realistic한 geometry를 갖도록 강제하였다.

==> 3_method_before.tex <==
%%%%%%%%% Notation
% 3D location: $\mathbf{x}$
% viewing direction: $\mathbf{d}$
% volume density : $\sigma$
% view-dependent RGB color : $\mathbf{c}$
% volume rendering function : $\pi$


% 차원 : \in \mathbb{R}^{3}


% -------------------------------------------------------------------------------

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/model_ex.png}
    \vspace{-0.2cm}
    \caption{Overview of a Model. }
    \vspace{-0.2cm}
    \label{fig:overview}
\end{figure*}

\section{Method}
\label{sec:method}
% 우리는 3D geometry-aware object generation문제를 풀고자 한다.
% Memory efficiency와 continuous한 representation의 장점을 얻기 위해 radiance field를 이용하여 3D를 표현함.
% View direction에 indepndent한 color (albedo)와 normal, specualr parameter를 예측한다.
% In this section, we exploit the main components of our method. % GIRAFFE
In this section, we present how we achieve to generate volume representations with realistic geometry along with realistic multi-view image generation.
First, we briefly review Neural Radiance Fields (NeRF) and volume rendering (Sec.~\ref{sec:preliminaries}).
Afterward, we explore our proposed method and how we render images (Sec.~\ref{sec:architecture}).
Third, we elaborate training and inference procedures (Sec.~\ref{sec:procedure}).
Finally, we discuss the implementation details (Sec.~\ref{sec:details}).

\subsection{Preliminaries.}\label{sec:preliminaries}
\textbf{Neural Radiance Field.}
Radiance field is a continuous function that maps a 3D location $\mathbf{x} \in \mathbb{R}^{3}$ and a viewing direction $\mathbf{d} \in \mathbb{S}^{2}$ to volume density $\sigma \in \mathbb{R}^{+}$ and view-dependent RGB color value $\mathbf{c} \in \mathbb{R}^{3}$. % GIRAFFE
Inspired by NeRF~\cite{nerf}, following work~\cite{graf, giraffe} use multi-layer perceptron to represent this mapping function as
\begin{equation}
\begin{gathered}
    f(\mathbf{x}, \mathbf{d}) = (\sigma, \mathbf{c}), \\
    f_1(\mathbf{x}) = \mathbf{h}, \quad
    f_2(\mathbf{h}) = \sigma, \quad
    f_3(\mathbf{h}, \mathbf{d}) = \mathbf{c}.
    \label{eq:nerf_1}
\end{gathered}
\end{equation}
% \begin{equation}
%     f(\mathbf{x}, \mathbf{d}) = (\sigma, \mathbf{c}),
%     f_2 \circ f_1(\mathbf{x}) = \sigma,
%     f_3(f_1(\mathbf{x}), \mathbf{d}) = \mathbf{c}, 
%     \label{eq:nerf_1}
% \end{equation}
To represent non-Lambertian effects of color, $\mathbf{d}$ is concatenated with intermediate feature vector $\mathbf{h}$ and passed to an additional layer that outputs view-dependent RGB color.

\textbf{Volume Rendering.}
% GIRAFFE 동일
% For the sampled camera pose $\xi$, let ${\{\mathbf{x}_j\}^{N_x}_{j=1}}$ be sample points along the camera ray $\mathbf{d}$ for a given pixel $uv \in \Omega$ where $\Omega$ denotes the set of pixels in the image plane.
%  and the resolution of the image plane $U\times{V}$
With given sampled camera pose $\xi$, let ${\{\mathbf{x}_j\}^{N_x}_{j=1}}$ be the sampled points along the camera ray for a given pixel location $(u, v)\in\Omega$, where $\Omega$ indicates the set of pixel locations in the image plane, and $N_x$ denotes the number of sampled points in a camera ray.
% To calculate expected pixel color for a camera ray $\mathbf{r}$, the color $\mathbf{c}_r^i$ and volume density $\sigma_r^i$ of samples along $\mathbf{r}$ 
To calculate the expected color $\mathbf{c}_{uv}$ for each pixel location $(u, v) \in \Omega$, the non-parametric volume rendering function $\pi_{vol}(\cdot)$ that maps the color $\mathbf{c}_j$ and the volume density $\sigma_j$ of the sampled point $\mathbf{x}_j$ to $\mathbf{c}_{uv}$ can be define as
% To calculate the expected color $\mathbf{c}_{uv}$ for each pixel location $(u, v)$, the non-parametric volume rendering function $\pi_{vol}(\cdot)$ thatcan be define as
% $\mathbf{c}_{uv}$ can be defined as
\begin{equation}
\pi_{vol}: (\mathbb{R}^+, \mathbb{R}^3)^{N_x} \rightarrow \mathbb{R}^3, \quad \{\sigma_j, \mathbf{c}_j\}^{N_x}_{j=1} \mapsto \mathbf{c}_{uv}.
\end{equation}
To be specific, we obtain the estimated color $\mathbf{c}_{uv}$ with numerical integration~\cite{nerf} as
\begin{equation}
\begin{gathered}
    \vspace{-0.3cm}
    % \pi_{vol}(\{\sigma_j, \mathbf{c}_j\}^{N_x}_{j=1}) = \sum_{j=1}^{N_x} w_j \mathbf{c}_j, \\
    \mathbf{c}_{uv} = \sum_{j=1}^{N_x} w_j \mathbf{c}_j, \quad
    w_j = \tau_j \alpha_j, \\
    \tau_j = \prod_{k=1}^{j-1}(1-\alpha_k), \quad
    \alpha_j = 1 - e^{-\sigma_j \delta_j},
    \vspace{-0.1cm}
    \label{eq:volume_rendering}
\end{gathered}
\end{equation}
% \begin{equation}
%     \mathbf{c}_r = \pi(\{\mathbf{c}_r^t, \sigma_r^t\}_{t=1}^{N})
%     \label{eq:volume_rendering}
% \end{equation}
where $\tau_j, \alpha_j$ denote the transmittance and the alpha value for $\mathbf{x}_j$, and $\delta_j=||\mathbf{x}_{j+1} - \mathbf{x}_j||_2$ is the L2-distance between the adjacent sampled points.

% shjung13: Please revisit here
To this end, we extend this definition to the volume parameter $\mathbf{p}$, which can be one of our novely-defined volume representations such as albedo $\mathbf{a}$, normal $\mathbf{n}$, and specular coefficients $\mathbf{sp}$, similar to Boss~\etal~\cite{nerd}.
The volume representations baked from our network are volume rendered as 
\begin{equation}
\begin{gathered}
    \vspace{-0.3cm}
    \mathbf{p}_{uv} = \sum_{j=1}^{N_x} w_j \mathbf{p}_j, \quad
    w_j = \tau_j \alpha_j. \\
    \vspace{-0.1cm}
    \label{eq:volume_rendering}
\end{gathered}
\end{equation}

\subsection{Generative Factorized Radiance Fields}\label{sec:architecture} %Generative Representation 
\textbf{Photometric Generative NeRF.}
Schwarz~\etal~\cite{graf} proposed a NeRF-based generative method that conditions the model on the latent code $z$, formulated as follows: $G(\mathbf{x}, \mathbf{d}, \mathbf{z}) = (\sigma, \mathbf{c})$.
% Similar to this, our model generates an implicit radiance filed which maps 3D location to color and density conditioned on $\mathbf{z}$.
The model generates implicit radiance field that maps a 3D location and view direction to density and color conditioned on $\mathbf{z}$.
Although recent approaches~\cite{giraffe, pigan} adopted the same scheme for their architecture, we find out this scheme can have following limitations. 
First, view-dependent color prediction can aggravate the quality of geometry since the model can generate photo-realistic images without well-formed geometry.
Moreover, they cannot explicitly control the light (\textit{i.e.,} changing light direction or intensity), which plays an essential role for identifying the defects of the geometry as illustrated in Fig.~\ref{fig:intro_sphere}.
% view dependent color --> non lambertian 나타내기 위해 --> specular, normal, albedo로 대체 --> light disentangle 가능 + introduction설명처럼 pred normal을 통해 arbitrary 한 light에서 realistic한 geometry를 업데이트 가능
% neural network에 non-lambertian effects (i.e., view-point에 의한 light reflection)을 예측하도록 지금까지 했다면, 이제는 명시적으로 light를 control하고 view-dependent한 color 대신 view-independent 한 color와 normal vector, 그리고 specular parameters를 예측해서 view point에 따른 빛의 reflection prior 통해 prediction함으로써 다양한 view point와 light에 대해 자연스러운 이미지를 생성해낼 수 있는 volume parameter들을 구해낼 수 있음. 또한, 이 구해진 parameter를 통해서 실제 생성된 implicit function의 geometry가 이러한 특성을 갖도록 강제하므로써 기존 모델에 대비 더욱 더 realistic한 geometry를 생성해낼 수 있도록 함.
To overcome these drawbacks coming from letting the neural networks learn the non-Lambertian effects by its own, we explicitly control the light and let the model predict the \textcolor{blue}{factorized volume representations, which are} view-independent albedo $\mathbf{a}$, normal vectors $\mathbf{n}$, and specular coefficients $\mathbf{sp}$, instead of view-dependent color. 
Afterward, we render the images via physical prior (\textit{i.e.,} photometric reconstruction with ambient, diffuse, and specular reflection) with obtained \textcolor{blue}{factorized volume representations}. 
% \textcolor{blue}{This novel architecture allows the model to learn }
\SH{Please revisit after intro} This novel architecture allows the model to predict the geometry property (\textit{i.e.,} normal vectors) that makes the images generated from various light and view point conditions realistic. 
In addition, with the obtained geometry property, we further regularize the volume geometry of implicit function to reflect it, achieving more realistic geometry than before.
Moreover, since we predict view-independent albedo through our model, we can predict albedo and density for every 3D location without sampling camera pose. 
This enables us to extract the textured mesh via marching cube algorithm from the generated volume representations, which is not possible for other previous work.
We will further illustrate this in the following paragraph.
% Therefore, we force the model to learn the neural radiance field excluding view directions and let the model predict density, albedo, normal, and specular parameters: $G(\mathbf{x}{x}, \mathbf{z}) = (\sigma, \mathbf{a}, \mathbf{n}, \mathbf{sp})$.
% The differences are that our model does not use view direction as the query and the output is composed of density, albedo, normal, and specular parameters: $G(\mathbf{x}, \mathbf{z}) = (\sigma, \mathbf{a}, \mathbf{n}, \mathbf{sp})$.\SH{Parameter? values?}
% This is elaborated in the later paragraph.
% view direction에 dependent하지 않은 것은 추후에 설명하겠음

% when --> for
Besides, we adopt the FiLMed SIREN architecture of Chan~\etal~\cite{pigan} as our main network, which leverages a mapping network for conditioning $\mathbf{z}$ and sinusoidal activation for \textcolor{blue}{improving} image quality.
As shown in Fig.x, the FiLMed SIREN is formulated as
\begin{equation}
\begin{split}
    \Phi(\mathbf{x}_j) = \phi_{n-1} \circ \phi_{n-2} \circ \mathellipsis \circ \phi_{0} ~ (\mathbf{x}_j), \\
    \phi_{i}(\mathbf{x}_j^{(i)}) = \sin (\boldsymbol{\gamma}_i \cdot (\mathbf{W}_i \mathbf{x}^{(i)}_j + \mathbf{b}_i) + \boldsymbol{\beta}_i),
        \label{eq:pigan_1}
\end{split}
\end{equation}
where $\phi_{i}$ denotes the $i^{th}$ FiLMed linear layer of the MLP followed by sinusoidal activation function, and $\mathbf{x}^{(i)}_j$ denotes the input vector of $\phi_{i}$.
$\boldsymbol{\gamma}^i$ and $\boldsymbol{\beta}^i$ denote the affine transformation parameters of FiLM layer~\cite{film}, which are the output of the mapping network conditioned on the latent vector $\mathbf{z}$.


\textbf{Factorized Volume Representations.}
% view dependent color나 모델이 light를 알고있는게 multiview에서 realistic하지만 unrealisitc한 geometry를 가질 수 있게하는 거 설명
In this paper, we explore representations based on photometric reconstruction, which enables the model to learn the physically correct geometry.
% photometric reconsturction 설명 들어가야할듯
As shown in Fig.~\ref{fig:overview}, we re-parameterize the view-dependent color output of previous methods~\cite{nerf, graf, pigan} with the normal $\mathbf{n}$, the specular coefficients $\mathbf{sp}$ and the view-independent color $a$ that is interpreted as albedo. 
Furthermore, to avoid degenerated solution where the model ignores the photometric reconstruction and places all responsibility on albedo, we use randomly sampled light conditions, which makes the model generate realistic images for arbitrary light conditions considering the photometric reconstruction.
The factorized volume representations, $\mathbf{a}\in\mathbb{R}^3$, $\mathbf{n}\in\mathbb{R}^3$, and $\mathbf{sp}\in\mathbb{R}^2$, of our model are defined as 
\begin{equation}
\begin{split}
    \sigma_{j} = \mathbf{W}_{\sigma}\Phi(\mathbf{x}_j) + \mathbf{b}_{\sigma}, \quad
    \mathbf{a}_{j} = \mathbf{W}_{a}\Phi(\mathbf{x}_j) + \mathbf{b}_{a}, \\
    \mathbf{n}_{j} = \mathbf{W}_{n}\Phi(\mathbf{x}_j) + \mathbf{b}_{n}, \quad
    \mathbf{sp}_{j} = \mathbf{W}_{sp}\Phi(\mathbf{x}_j) + \mathbf{b}_{sp},
    \label{eq:factorized}
\end{split}
\end{equation}
where $\mathbf{W}_{p}$ and $\mathbf{b}_{p}$ denote the weight and bias of the additional linear layer for volume parameter $\mathbf{p}$, and $\Phi(\mathbf{x}_j)$ is intermediate feature vector. 
$\mathbf{sp}$ consists of the specular relfection coefficient and the shineness coefficient.
%the two-dimensional specular parameters
% 인트로에서 쓴 이유처럼 조금더 부연설명 필요할 듯
% light sample하는거 설명
% To obtain factorized representation, we re-parameterize the output of NeRF with veiw-independent color and high dimensional feature $\mathbf{f}$ following GIRAFFE~\cite{niemeyer2021giraffe}.
% While GIRAFFE volume render $\mathbf{f}$ and use 2D CNN based neural rendering to upsample low resolution feature maps to higher-resolution RGB images, convolution operation between adjacent pixels on image plane hurts internal 3D-aware feature, which leads to multi view inconsistency and noisy geometry.
% Thus, we obtain the factorized representation by passing the volume rendered $\mathbf{f}$ to one additional Linear layer.
% \textbf{Factorized Representation.}
% % 여기서부터 GIRAFFE와 거의 비슷하게 쓴 것임
% For the sampled camera pose $\xi$, let ${\{\mathbf{x}_j\}^{N_x}_{j=1}}$ be sample points along the camera ray $\mathbf{d}$ for a given pixel $uv \in \Omega$ where $\Omega$ denotes the set of pixels in the image plane, and $(\sigma_j, \mathbf{a}_j, \mathbf{n}_j, \mathbf{sp}_j) = G(\mathbf{x}_j)$ the corresponding densities and factorized representation of the field. The volume rendering operator with numerical integration~\cite{nerf} maps these outputs to the pixel's final representation vector $\mathbf{f}_{uv}$:\SH{$\boldsymbol{f}$는 tensor이고, $\boldsymbol{f}_{u, v}$가 vector인가요?}
% \begin{equation}
% \begin{split}
%     \vspace{-0.3cm}
%     \mathbf{a}_{uv} = \sum_{j=1}^{N_s} w_j \mathbf{a}_j, \quad
%     \mathbf{n}_{uv} = \sum_{j=1}^{N_s} w_j \mathbf{n}_j, \quad
%     \mathbf{sp}_{uv} = \sum_{j=1}^{N_s} w_j \mathbf{sp}_j, \\
%     w_j = \tau_j \alpha_j, \quad
%     \tau_j = \prod_{k=1}^{j-1}(1-\alpha_k), \quad
%     \alpha_j = 1 - e^{-\sigma_j \delta_j},
%     \vspace{-0.3cm}
%     \label{eq:volume_rendering}
% \end{split}
% \end{equation}
% where $\tau_j$ is the transmittance, $\alpha_j$ is the alpha value for $\mathbf{x}_j$, and $\delta_j = ||\mathbf{x}_{j+1} - \mathbf{x}_j||_{2}$ is the distance between neighboring sample points.
% $\mathbf{n}$ denotes three-dimensional unit normal vector, $\mathbf{sp}$ denotes the two-dimensional specular parameters.
% With the volume rendered feature vector $\mathbf{f}$ as an input, the Linear layer outputs the factorized representation (\eg normal and specular parameters).
% \begin{equation}
%     \vspace{-0.3cm}
%     \mathbf{n} = Linear_n(\mathbf{f}), \quad (\mathbf{sp}^a, \mathbf{sp}^b) = Linear_{sp}(\mathbf{f}),
%     % \vspace{-0.3cm}
%     \label{final_linear}
% \end{equation}


Although the normal of the implicit function(\eg neural radiance field) at a point $j$ can be obtained by  $-\frac{\nabla_\textbf{x}\sigma_j}{\|\nabla_\textbf{x}\sigma_j\|}$~\cite{nerd, nerfactor, multiview}, utilizing this directly for the reconstruction can lead to sub-optimal results for following reasons.
% 이를 직접적으로 photometric reconstruction에 사용하여 sigma를 업데이트 하는 것은 다음과 같은 이유로 어렵다.
As also pointed out in zhang~\etal~\cite{nerfactor}, the gradient of volume density tends to be noisy, and this makes it difficult to render clear images when exploiting the gradient of $\sigma$ for rendering.
Moreover, since all the factored representations are dependent on $\sigma$ in volume rendering process, employing the gradient of $\sigma$ for the component of photometric reconstruction can cause unstable training.
% Also, 우리가 photometric reconstruction에 사용하는 모든 components (\eg, albedo, specular, etc)은 sigma에 의해서 volume rendering 되기 때문에, sigma의 gradient를 normal로 사용하는 것은 학습을 불안정하게 만든다.
% the gradient of the sigma tends to be noisy, which makes it hard to use this normal as the component of photometric reconstruction.
Thus, we induce an additional prediction branch to estimate the normal $\mathbf{n}_j$ at the point $j$ and use the output (\textit{i.e.,} predicted normal) as the component of photometric reconstruction. 
% where MSE loss aligns the predicted normal and TV loss reduces the variance.
As a consequence, we are able to stably disentangle the view-dependent color into albedo, specular coefficients, and normal while satisfying realistic photometric reconstruction under arbitary light conditions.
To further refine the geometry of the generated volume representations, we utilize this predicted normal for the guidance of the gradient of $\sigma$. Integrating this with total variation (TV) loss to smooth out the normal in the local region, our normal loss is defined as 
% Also, we can use the predicted normal as the weak supervision to the gradient of $\sigma$, which refines the geometry of the generated volume representations. 
% \begin{equation}
\begin{flalign}
\begin{split}
    % L_\text{Normal} = \text{MSE}\left(\textbf{n}_{pred}, -\frac{\nabla_\textbf{x}\sigma}{\|\nabla_\textbf{x}\sigma\|}\right) + k L_\text{TV}\left(\textbf{n}_{pred}\right)
    \vspace{-0.3cm}
    &L_\text{Normal} =\\
    &\sum_{(u,v) \in \Omega} \bigg\{ \sum_{j=1}^{N_x} w_j  ||\mathbf{n}_{j} - \frac{\nabla_\mathbf{x}\sigma_j}{\|\nabla_\mathbf{x}\sigma_j\|_2} 
    ||_{2}
    + \lambda L_\text{TV}\left(\mathbf{n}_{uv}\right)
    \bigg\}.
    \label{normalloss}
    \vspace{-0.3cm}
\end{split}
\end{flalign}
% \end{equation}
In previous 3D-aware image generation work, the models are trained only with 2D GAN loss, which does not focus on the reality of internal geometry.
However, since our model tries to achieve the realistic photometric reconstruction with the predicted normal and use it as the weak supervision of the geometry, the geometry can be refined to be more smooth and realistic.
% the model can optimize the $\sigma$.
% Thus, the geometry is refined to be smoothed and realistic.
% During the output of the normal branch and the gradient of the sigma follow each other, the following advantages can be obtained.
% shjung13: removes the noise from the gradient of the sigma and obtain a more robust and representative one 
% First, we encourage the predicted normal to play a role of the normal.
% Without the regularization that enforces the predicted normal to follow the gradient of the sigma, the model falls into the degenerate solutions where the photometric reconstruction is ignored.
% Next, the geometry of the generated implicit function is refined by providing weak supervision to the gradient of $\sigma$.
% In previous work, models are trained only with 2D GAN loss, which does not focus on the reality of internal geometry.
% However, since our model tries to achieve the realistic photometric reconstruction with the predicted normal, it can be used as the weak supervision of the gradient of $\sigma$.
% By optimizing the $\sigma$ in the second order gradients with the supervision, the geometry is refined to be smoothed and realistic.
% shjung13: empirically --> smooth out the normal vectors in the local region

% 2D GAN loss로만 학습하기 때문에 geometry를  

% 우리가 빼준 브랜치가 normal의 역할을 하도록 강제하기 위해 일단 noisy 하더라도 model normal을 따라가게 하고 (unsupervised 상황에서도) photometric image rendering시 이 normal로 진행
% 근데 이렇게만하면 예측 normal noisy해질 수 있으므로 tv로스도 걸어주고
% + discriminator loss로 이렇게 잘 예측된 normal을 

% 의 upper bound가 원래 unrealistic geometry 로 정해질 수 있다
% 그래서 우리는 이 realistic하게 예측된 예측 normal을 기반으로 model normal을 update해주고, 이는 sigma에 second order gradient를 흘려서 geometry를 realistic하게 개선시킨다.


\textbf{Photometric Image Rendering.}
% shjung13: Equation으로 식 변경
% shjung13: scalar, vector notation, shape 명시
The final textured image is rendered from a combination of albedo, normal, specular coefficients, light, and view direction.
% shjung13: Gaussian?
We sample light $l=(k_a, k_d, l_d)$ from the prior distribution, where $l$ consists of the intensity of ambient light $k_a\in\mathbb{R}^{+}$, the intensity of directional light $k_d \in \mathbb{R}^{+}$, and the direction of light $l_d \in \mathbb{R}^3$.
% shjung13: directional illumination == shading map? "obtain a value" --> notation
We calculate the dot product of the normal $n_{uv}$ and light direction $l_d$ to obtain a value for the directional illumination.
Afterward, the shading map $\mathbf{S}$ is obtained by multiplying the intensity of directional light and adding the intensity of ambient light to the obtained value: $\mathbf{S}_{uv} = (k_a + k_d \cdot max\{0, \langle l_d, n_{uv} \rangle \})$.
The specular map $\mathbf{SP}$ is obtained from the predicted specular coefficients, the normal, the directional light and the view direction, as follows:  $\mathbf{SP}_{uv} = k_d \cdot \mathbf{sp}^{(0)}_{uv} \cdot (max\{0, \cos \theta\})^{\mathbf{sp}^{(1)}_{uv}}$, where $\theta$ denotes the angle between the view direction and the reflected light direction by the normal, and $\mathbf{sp}^{(0)}, \mathbf{sp}^{(1)}$ denote the specular reflection coefficient and shineness coefficient, respectively.
% $i$-th channel of $\mathbf{sp}$.
% shjung13: \textit{i.e.,} non-Lambertial effects?
% Note that the specular map represents the view-dependent color change (non-Lambertian effects).
Note that this process is calculated for each pixel $(u, v)$ in the image plane.
Finally, we render the final textured image from a combination of albedo, shading map, and specular map, formulated as
\begin{equation}
% \begin{gathered}
\mathbf{I} = \mathbf{a} \cdot \mathbf{S} + \mathbf{SP}.
% \end{gathered}
\end{equation}
% , I = \{I_{uv}\}_{uv\in{\Omega}}$.

\subsection{Training and Inference}\label{sec:procedure}

\textbf{Training Loss.}
Fig.~\ref{fig:overview} depicts the overall training procedure.
Our model first samples a latent variable $\mathbf{z} \sim \mathcal{N}(0, \mathbf{I})$ to condition the model.
We sample points $\{\textbf{x}_{j=1}\}_j^{N_x}$ on the ray direction drawn by a random camera pose $\xi \sim p_\xi$ and sample the random light condition $l \sim p_l$. 
%of which $p_\xi$ is obtained by estimating the data prior.
% On the first stage of our training procedure, the model $G$ is trained by the same way with pi-gan~\cite{pigan}, optimizing the rough volume density $\sigma$ and the color $\textbf{c}$.
% On the second stage, our model $G$ outputs $(\sigma_j, \textbf{a}_j, \textbf{f}_j)$ as well as $\textbf{c}_j$.
% We leverage the gathered $\{\sigma_j\}_j^{N_x}$ to calculate the point weights $\{\textbf{w}_j\}_j^{N_x}$, obtain $\textbf{a}_{uv}$ and $\textbf{f}_{uv}$ by volume-rendering, and estimate $(n_{uv}, \textbf{sp}^a, \textbf{sp}^b)$ by linear projection on $\textbf{f}_{uv}$.
% To render a photometric image, we sample light parameters $(k_a, k_d)$ and light direction $l$, and then tint the albedo $\textbf{a}_{uv}$ with the estimated shading $\textbf{S}_{uv}$ and specular $\textbf{SP}_{uv}$, generating the final output image.
Then, we train our model $G_\theta$ using the non-saturating GAN~\cite{gan} loss with R1 regularization~\cite{r1_regularization}:
\begin{equation}
\begin{split}
    \vspace{-0.3cm}
    L_\text{GAN}(\theta, \phi) = \mathbf{E}_{\mathbf{z} \sim p_z, \xi \sim p_\xi, l \sim p_l}[f(D_{\phi}(G_{\theta}(\mathbf{z}, \xi, l)))] \\
    + \mathbf{E}_{I \sim  p_D}[f(-D_{\phi}(I)) 
    - \lambda \|\nabla D_{\phi}(I)\|^{2}],
    \vspace{-0.3cm}
\label{GANloss}
\end{split}
\end{equation}
where $f(x) = -log(1 + exp(-x))$, $p_D$ denotes the real data distribution, and $D_{\phi}$ indicates the discriminator.
$D_{\phi}$ is trained by maximizing Eq.~\eqref{GANloss}, and the generator is trained by minimizing both Eq.~\eqref{normalloss} and Eq.~\eqref{GANloss}: 
\begin{equation}
    L_{total} = L_{GAN} + \lambda_{n}L_{normal},
\end{equation}
where $\lambda_{n}$ denotes the hyper-parameter indicating the relative importance between two losses.

% \textbf{Staged training.}
% To accelerate the training, we adopt the pretrained pi-gan.

\textbf{Inference.}
% Image generation process is the same to the training process.
Through our novel architecture, we can take two main advantages as follows:
1) We can generate re-lightable images since we disentangle the light conditions and factorize the texture into albedo, normal, and specular coefficients.
We can generate the images with arbitrary light conditions and view points where we want to render the images from.
% For the desired light condition and the view point, we can render the image as $G_\theta(\mathbf{z}, \xi, l)$.

2) We also can extract the textured mesh from generated volume representations.
First, we can extract the surface points via marching cube algorithm on the volume density of generated representations.
Next, since the model predicts the volume representations independent from viewing direction, we can obtain the albedo and the specular coefficients of the surface points.
With these obtained textured mesh with the albedo and specular coefficients, we can relight the mesh using 3D rendering tools such as Blender.
This is a significant improvement for applications such as games or movies since those applications require the texture of mesh that does not contain the light in its color.
To be more specific, the textured mesh has to be rendered with various light conditions in 3D space, and if there still remains the effect of light in the texture, the rendered scene would be unnatural.

To the best of our knowledge, ours is the first among generative models not requiring additional label or assumptions (\eg assumption of symmetric or ellipsoid object) and capable of generating re-lightable images and textured meshes with unposed 2D images alone.
% Moreover, we are the first approach that is able to generate textured mesh among generative models.

% Since we predict view-independent albedo and utilize disentangled light conditions, we are able to generate textured mesh and re-lightable images. Furthermore, we can again re-l
% textured mesh / relighting
% 이미지 generation은 training 과정과 동일.
% l을 다양하게 해서 rendering하면 re-lightable image.
% The ability to extract a textured mesh is one of the key advantages of the our method. % (NeRD)
% This is not possible with previous NeRF-based generation methods where the color is predicted depending on the view direction. % (NeRD)

% \textbf{Discriminator.}

\subsection{Implementation details}\label{sec:details}





% \textbf{Photometric Generative Network.}
% In this paper, we explore photometric reconstruction-based representation which enables the model to learn the physically correct geometry.
% As shown in Fig.~\ref{fig:overview}, we replace the view-dependent color output of previous methods~\cite{mildenhall2020nerf, schwarz2020graf, chan2021pi} with the normal, the specular parameters and the view-independent color which is interpreted as albedo. 
% To avoid degenerated solution where the model ignores the photometric reconstruction and places all responsibility on albedo, we use randomly sampled light conditions, which makes the model try to generate realistic images for arbitrary light conditions considering the photometric reconstruction.

% To obtain factorized representation, we re-parameterize the output of NeRF with veiw-independent color and high dimensional feature $\mathbf{f}$ following GIRAFFE~\cite{niemeyer2021giraffe}.
% While GIRAFFE volume render $\mathbf{f}$ and use 2D CNN based neural rendering to upsample low resolution feature maps to higher-resolution RGB images, convolution operation between adjacent pixels on image plane hurts internal 3D-aware feature, which leads to multi view inconsistency and noisy geometry.
% Thus, we obtain the factorized representation by passing the volume rendered $\mathbf{f}$ to one additional Linear layer.

% \textbf{Factorized Representation.}
% For the sampled camera pose $\xi$, let ${\{\mathbf{x}_j\}^{N_x}_{j=1}}$ be sample points along the camera ray $\mathbf{d}$ for a given pixel $uv$, and $(\sigma_j, \mathbf{a}_j, \mathbf{f}_j) = G(\mathbf{x}_j)$ the corresponding densities and feature vectors of the field. The volume rendering operator with numerical integration~\cite{mildenhall2020nerf} maps these evaluations to the pixel's final feature vector $\mathbf{f}_{uv}$:\SH{$\boldsymbol{f}$는 tensor이고, $\boldsymbol{f}_{u, v}$가 vector인가요?}

% \begin{equation}
% \begin{split}
%     \vspace{-0.3cm}
%     \mathbf{a}_{uv} = \sum_{j=1}^{N_s} w_j \mathbf{a}_j, \quad
%     \mathbf{n}_{uv} = \sum_{j=1}^{N_s} w_j \mathbf{n}_j, \quad
%     \mathbf{sp}_{uv} = \sum_{j=1}^{N_s} w_j \mathbf{sp}_j, \\
%     w_j = \tau_j \alpha_j, \quad
%     \tau_j = \prod_{k=1}^{j-1}(1-\alpha_k), \quad
%     \alpha_j = 1 - e^{-\sigma_j \delta_j},
%     \vspace{-0.3cm}
%     \label{eq:volume_rendering}
% \end{split}
% \end{equation}
% where $\tau_j$ is the transmittance, $\alpha_j$ is the alpha value for $\mathbf{x}_j$, and $\delta_j = ||\mathbf{x}_{j+1} - \mathbf{x}_j||_{2}$ is the distance between neighboring sample points.
% $\mathbf{n}$ denotes three-dimensional unit normal vector, $\mathbf{sp}^a$ \~, and $\mathbf{sp}^b$ \~.

